Contribution Evaluation in Federated Learning: Examining Current Approaches

Federated Learning (FL) has seen increasing interest in cases where entities want to collaboratively train models while maintaining privacy and governance over their data. In FL, clients with private and potentially heterogeneous data and compute resources come together to train a common model without raw data ever leaving their locale. Instead, the participants contribute by sharing local model updates, which, naturally, differ in quality. Quantitatively evaluating the worth of these contributions is termed the Contribution Evaluation (CE) problem. We review current CE approaches from the underlying mathematical framework to efficiently calculate a fair value for each client. Furthermore, we benchmark some of the most promising state-of-the-art approaches, along with a new one we introduce, on MNIST and CIFAR-10, to showcase their differences. Designing a fair and efficient CE method, while a small part of the overall FL system design, is tantamount to the mainstream adoption of FL.

==> incentive_mechs.tex <==
The concept of fairness in a FL process extends beyond the design of the CE function that maps actors to their value/worth. Whereas that is only a problem of conceptualising and efficiently calculating a fair value, the overall system model has to account for various other considerations, such as the costs participants occur to collect data, or participants being self-interested and thus interested in maximising their payoff while minimising their costs, even by not collecting high quality data or misreporting it, among others. This problem of designing a FL system that \textit{incentivizes} participants to truthfully participate, is called \textit{Incentive Mechanism Design}. Because of the broader scope of IMD compared to CE, the related works are more heterogeneous; most of the works do not explicitly search for an \textit{a priori} fair payoff allocation, but rather an \textit{a posteriori} one since the participants are incentivized to truthfully participate in the federation. We follow \cite{huang_exploratory_2020} in defining, in a relatively straight-forward manner, IMD for FL as:
\begin{defn}
"Incentive Mechanism of Federated Learning: An incentive mechanism in FL system consists of a set of rewards $R$ and three functions $v$, $c$, and $r$. The function $v: R \to \R$ assigns each reward a value. For a set of participants $P$, the function $c : P \to \R$ assigns each participant a score that measures their contribution to the system ... Last, the function $r : R \to \R$ assigns a reward based on the score that $c$ provides. The reward function $r$ offers rewards of monotonously increasing value, i.e., if $x > y$, then $(r(x)) \ge (r(y))$."
\end{defn}

Cong et al.\cite{Cong2020} provide a very comprehensive game-theoretic framework for IMD that accounts for different sources of untruthfulness such as misreporting costs or data. They propose splitting the problem into a supply-side problem, where the server tries to optimally select the best participants at each round and allocate payments to them, and a demand-side, where each participant tries to coax the best possible payment and access to the model, and propose the Crémer-McLean mechanism and a procurement auction, respectively, to model those. 

Kang et al.\cite{kang_incentive_2019} presented an IMD for case of cross-device FL, where \textit{reputation} is used as a measure of data quality: when each participant joins in on a task, his contributions, if of high quality, count towards increasing his reputation on a blockchain-based ledger. Each new central orchestrator can view the reputations of all devices and select only the ones with a high reputation score. One problem with this approach is it assumes devices will participate in many tasks, and, most importantly, that if a device performed in a certain way for one task it will do so for another. 

As is correctly pointed out by Yu et al.\cite{yu_sustainable_2020}, there is a practical issue of a delay between when an actor makes a contribution, and when he gets rewarded by it, as it takes time to train and deploy any ML model. Their main goal is thus to address this temporal mismatch between actors contributing to the federation and the federation generating the necessary profit to pay them back, by designing a dynamic budget allocation algorithm. Of note is the fact their IMD is independent of both the evaluation contribution and the cost calculation methods, allowing for more flexibility. The difference between these two quantities is the \textit{regret} of each participant, i.e. the debt the federation owes them. They formulate the problem of stabilising the federation as one of minimising the accumulated, over time, regret of each participant, while maximising the collective utility of the federation. This is equivalent to maximising a "value-minus-regret-drift" objective over time, which can be modeled by a linear program solvable in $O(N)$. The solution is the reward each participant is owed by the federation at every time step. 

Richardson et al.\cite{Richardson2020} present an IMD based on the cumulative influence of each participant's datapoints. Using influence functions as incentives improves upon the SV by taking, by construction, the order of data into account: it motivates early participation (as earlier updates are more influential than later ones) and assigns a zero rewards to redundant data. They show that this IMD can elicit truthful participation, under a bounded payoff budget, even when considering the costs clients incur to gather data. But the influence function, which we remind is an asymptotic approximation of sample-level LOO, has (so far in FL) only been approximated\cite{influence_aprox} under the assumptions of monotonically decreasing risk and the ability to calculate the model's Hessian, meaning, practically, this IMD is only of interest for simple underlying models like linear and logistic regression. 

Recently, Hasan\cite{hasan2021incentive} expanded beyond the common assumption of the grand coalition forming, by instead examining the incentives necessary to stabilise smaller coalitions under (Nash) stability and \textit{hedonic games}. In a hedonic game the participants have preferences over which players they want to collaborate with; as a real-world example, you might not want to collaborate with your biggest competitor but are fine with everyone else. He shows that under this setting it is possible for an imputation under the solution concept of the Nash-stable set to exist, i.e. the set can be non-empty, but checking for a solution is NP-Hard.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
{ % begin box to localize effect of arraystretch change
\renewcommand{\arraystretch}{1.5}
\begin{table*}[h]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|l|c|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
{\ul \textbf{Participants}} &
  \multicolumn{5}{c|}{\textbf{2}} &
  \multicolumn{5}{c|}{\textbf{4}} &
  \multicolumn{5}{c|}{\textbf{6}} &
  \multicolumn{5}{c|}{\textbf{8}} &
  \multicolumn{5}{c|}{\textbf{10}} \\ \hline
\multicolumn{1}{|c|}{} &
  \textbf{Acc} &
  \multicolumn{1}{c|}{\textbf{Max Dif}} &
  \multicolumn{1}{c|}{\textbf{Dist}} &
  \multicolumn{1}{c|}{\textbf{t}} &
  \multicolumn{1}{c|}{\textbf{B}} &
  \multicolumn{1}{c|}{\textbf{Acc}} &
  \multicolumn{1}{c|}{\textbf{Max Dif}} &
  \multicolumn{1}{c|}{\textbf{Dist}} &
  \multicolumn{1}{c|}{\textbf{t}} &
  \multicolumn{1}{c|}{\textbf{B}} &
  \multicolumn{1}{c|}{\textbf{Acc}} &
  \multicolumn{1}{c|}{\textbf{Max Dif}} &
  \multicolumn{1}{c|}{\textbf{Dist}} &
  \multicolumn{1}{c|}{\textbf{t}} &
  \multicolumn{1}{c|}{\textbf{B}} &
  \multicolumn{1}{c|}{\textbf{Acc}} &
  \multicolumn{1}{c|}{\textbf{Max Dif}} &
  \multicolumn{1}{c|}{\textbf{Dist}} &
  \multicolumn{1}{c|}{\textbf{t}} &
  \multicolumn{1}{c|}{\textbf{B}} &
  \multicolumn{1}{c|}{\textbf{Acc}} &
  \multicolumn{1}{c|}{\textbf{Max Dif}} &
  \multicolumn{1}{c|}{\textbf{Dist}} &
  \multicolumn{1}{c|}{\textbf{t}} &
  \multicolumn{1}{c|}{\textbf{B}} \\ \hline
\textbf{OR - Shapley} &
  \multirow{2}{*}{0.84} &
  0.62 &
  0.44 &
  \multirow{2}{*}{\textbf{653}} &
  0.71 &
  \multirow{2}{*}{0.78} &
  0.46 &
  0.34 &
  \multirow{2}{*}{\textbf{687}} &
  0.68 &
  \multirow{2}{*}{0.73} &
  0.42 &
  0.34 &
  \multirow{2}{*}{863} &
  0.63 &
  \multirow{2}{*}{0.68} &
  0.46 &
  0.42 &
  \multirow{2}{*}{1510} &
  0.55 &
  \multirow{2}{*}{0.62} &
  0.46 &
  0.43 &
  \multirow{2}{*}{4186} &
  0.53 \\ \cline{1-1} \cline{3-4} \cline{6-6} \cline{8-9} \cline{11-11} \cline{13-14} \cline{16-16} \cline{18-19} \cline{21-21} \cline{23-24} \cline{26-26} 
\textbf{OR - LC} &
   &
  0.31 &
  0.22 &
   &
  0.84 &
   &
  0.41 &
  0.33 &
   &
  0.78 &
   &
  0.3 &
  0.24 &
   &
  0.73 &
   &
  0.23 &
  0.22 &
   &
  0.68 &
   &
  0.17 &
  0.21 &
   &
  0.62 \\ \hline
\textbf{LOO no weights} &
  \multirow{3}{*}{0.837} &
  \textbf{0.94} &
  \textbf{0.66} &
  \multirow{3}{*}{683} &
  1.4 &
  \multirow{3}{*}{0.78} &
  \textbf{0.55} &
  \textbf{0.41} &
  \multirow{3}{*}{717} &
  1.4 &
  \multirow{3}{*}{0.74} &
  0.38 &
  0.34 &
  \multirow{3}{*}{\textbf{760}} &
  1.1 &
  \multirow{3}{*}{0.68} &
  0.33 &
  0.33 &
  \multirow{3}{*}{\textbf{782}} &
  1.05 &
  \multirow{3}{*}{0.65} &
  0.35 &
  0.4 &
  \multirow{3}{*}{\textbf{819}} &
  0.68 \\ \cline{1-1} \cline{3-4} \cline{6-6} \cline{8-9} \cline{11-11} \cline{13-14} \cline{16-16} \cline{18-19} \cline{21-21} \cline{23-24} \cline{26-26} 
\textbf{LOO lin. weights} &
   &
  0.74 &
  0.52 &
   &
  6.1 &
   &
  0.47 &
  0.35 &
   &
  5.84 &
   &
  0.31 &
  0.27 &
   &
  4.6 &
   &
  0.29 &
  0.27 &
   &
  4.3 &
   &
  \textbf{0.29} &
  \textbf{0.32} &
   &
  2.9 \\ \cline{1-1} \cline{3-4} \cline{6-6} \cline{8-9} \cline{11-11} \cline{13-14} \cline{16-16} \cline{18-19} \cline{21-21} \cline{23-24} \cline{26-26} 
\textbf{Reputation} &
   &
  0.25 &
  0.17 &
   &
  1.6 &
   &
  0.11 &
  0.1 &
   &
  3.4 &
   &
  0.125 &
  0.14 &
   &
  4.8 &
   &
  0.17 &
  0.16 &
   &
  5.8 &
   &
  0.14 &
  0.16 &
   &
  7 \\ \hline
\textbf{$\lambda$-MR} &
  \multicolumn{1}{l|}{\multirow{2}{*}{0.832}} &
  0.29 &
  0.2 &
  \multirow{2}{*}{880} &
  3.3 &
  \multirow{2}{*}{0.78} &
  0.46 &
  0.35 &
  \multirow{2}{*}{1130} &
  3.4 &
  \multirow{2}{*}{0.74} &
  0.48 &
  \textbf{0.4} &
  \multirow{2}{*}{2116} &
  3.36 &
  \multirow{2}{*}{0.67} &
  \textbf{0.5} &
  \textbf{0.46} &
  \multirow{2}{*}{5000} &
  3.36 &
  \multirow{2}{*}{-} &
  - &
  - &
  \multirow{2}{*}{-} &
  - \\ \cline{1-1} \cline{3-4} \cline{6-6} \cline{8-9} \cline{11-11} \cline{13-14} \cline{16-16} \cline{18-19} \cline{21-21} \cline{23-24} \cline{26-26} 
\textbf{Federated Shapley} &
  \multicolumn{1}{l|}{} &
  0.3 &
  0.21 &
   &
  3.2 &
   &
  0.45 &
  0.34 &
   &
  2.9 &
   &
  \textbf{0.49} &
  \textbf{0.4} &
   &
  2.62 &
   &
  \textbf{0.5} &
  \textbf{0.46} &
   &
  2.28 &
   &
  - &
  - &
   &
   \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Results on CIFAR-10; Acc is the global model accuracy. Max Dif is the maximum distance between elements of the payoff vector. Distance refers to the Euclidean distance from the corresponding uniform vector. The time t is given in seconds. B is the total budget allocated by the un-normalised payoffs, and the only metric calculated before they are normalised. }
\label{tab:cifar_results}
\end{table*}}

==> intro.tex <==
In recent years, machine learning has become the driving force behind many key scientific breakthroughs. With the computational efficiency of our hardware being as high as it is, the key bottleneck in most real-world applications is the availability of data. Our data collection capabilities have also increased as more and more of our everyday devices, even vehicles, become connected. But with that has come increased public awareness and regulatory scrutiny about the value of privacy. As our societies move towards implementing stronger privacy-protection laws such as GDPR\cite{GDPR}, public companies are forced to follow suit in protecting their users against their data being unwillingly harvested\cite{applefb,googlecookies}.

At the same time as this push for privacy is taking place, technology companies are becoming more adept at leveraging personal data to improve their products and services, despite their customers becoming increasingly more hesitant about handing over their raw data. This same antithesis can be found in Medical ML/AI for Healthcare, where care providers are bound by law to protect the privacy of patients' health records but those could be used to train better automated diagnosis systems, potentially saving lives. So a solution that would allow private data to be used for training ML systems, while not compromising the owners' privacy, seems necessary.

Federated Learning\cite{mcmahan2017communicationefficient} was conceived as such a machine learning paradigm, where clients, usually orchestrated by a central entity, can collaborate without sharing their raw data with anyone, by instead transmitting updates to the central server, which are in turn aggregated to improve a global model. Besides alleviating the concerns of the end-users, i.e. citizens who are reluctant to hand over identifying information to corporations, Federated Learning opens up a path for the formation of consortia between competing companies. Under privacy guarantees, as long as the global model is better than the individual models of the companies, it is potentially to their benefit to be a part of the Federation. 

In both cases, i.e. when the potential FL clients are end-users, e.g. mobile devices collaborating to improve next word prediction in a keyboard app, and also when they are organisations, e.g. hospitals training a joint medical image segmentation models, the orchestrator has to overcome their \textit{reluctance} to share data, even in the form of updates. In the latter case, collecting, labeling, and curating a dataset comes with significant procurance costs. Even in the former case of end-users, the data is of a personal nature and users might be unwilling to altruistically share it, even if given theoretical privacy guarantees.

Other design considerations are how the objectives of the federation are balanced (e.g. between maximising global model accuracy and fairness) or how to model the \textit{information asymmetry}\cite{Cong2020} between what the participants report their data curation costs or even their datasets themselves to be, and what they really are. As an example, a poorly designed compensation scheme might incentivize strong participant(s) to hold-out their best data from what they present to the federation, or misreport their curation costs to garner higher rewards. 

A \textit{payoff scheme} that guarantees each actor will be compensated in fair proportion to her contributions, is necessary to convince participants to join the Federation. While much work has focused on how to value data, treating data as a commodity, and creating data marketplaces, the less-examined FL setting introduces new challenges which this report aims to highlight.

The goal of this report is to: 
\begin{itemize}
\setlength\itemsep{0.05em}
\item Introduce readers to relevant background knowledge on Federated Learning and Game Theory.
\item Agglomerate and classify the relevant literature in Data Evaluation, Contribution Evaluation in FL, and Incentive Mechanism Design in a manner that promotes building upon existing ideas.
\item Produce a novel, fair, and reproducible empirical comparison of promising state-of-the-art, as well as one we derive ourselves, Contribution Evaluation methods, examined on large-scale datasets, and make the code publicly available to foster research.
\item Discuss the open problems and potential areas of improvement on this topic.
\end{itemize}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/IMG_F0A05B9AFE0D-1.jpeg}
    \caption{Client-server FL model. Figure adapted from \cite{yang_federated_2019}}.
    \label{fig:flfig}
\end{figure}
